Hyperbolicity of singular spaces

We study the hyperbolicity of singular quotients of bounded symmetric domains. We give effective criteria for such quotients to satisfy Green-Griffiths-Lang's conjectures in both analytic and algebraic settings. As an application, we show that Hilbert modular varieties, except for a few possible exceptions, satisfy all expected conjectures.

==> cyclic.tex <==
\section{Cyclic quotient singularities}\label{sing}

In this section, we collect some basic facts about cyclic quotient singularities.
\subsection{Resolution}
First, we recall how one can resolve this type of singularities. This problem has been adressed by Fujiki (\cite{fu}).

Let $G$ a finite cyclic group with a fixed generator acting on a complex affine $m$-space ${\C}^ m={\C}^m(z_1,...,z_m)$ by the formula:

$$g(z_1,..,z_m)=(e_1 z_1,...,e_m z_m)$$

where, for each $i$, $e_i$ is a $n^{th}$ root of the unity, $n>1$. Then the quotient $X={\C}^m/G$ has the structure of a normal affine algebraic variety whose singular locus is reduced to the single point $p=\pi (0)$ where $\pi:{\C}^m\rightarrow X$ denotes the canonical projection.

Following \cite{fu} (theorem 1 p.303) there exists a resolution of the singularity of $X$, that is a pair $(\tilde X, f)$ consisting of a smooth variety $\tilde X$, a proper birational morphism $f:\tilde X \rightarrow X$ isomorphic outside $f^{-1} (p)$ with the additional following properties 

\begin{enumerate}
 \item $E=f^{-1} (p)$ is a simple normal crossing hypersurface, each component of which being rational.

\item There exists an affine open covering $\mathcal U=(U_1,...,U_l)$ of $\tilde X$ with $U_i\simeq{\C}^m$.

\item $f^{-1}(p)\cap U_i$ is defined by $u_{k_1}^i...u_{k_t}^i=0$ in $U_i\simeq {\C}^m(u^i)$ for some $k_1,..,k_t$ (depending on $i$) if it is non empty.

\item For each $i$ the multivaluate map $f\circ \pi:{\C}^m (u^i)\rightarrow {\C}^m(z)$ takes the following form:
 \begin{equation}\label{exprcoord}
z_k=\prod_{l=1}^m {u_l^i}^{b_{lk}}
\end{equation}

where $b_{lk}$ are nonnegative rational numbers (depending on $i$ and stricly less than $1$).
\end{enumerate}

\begin{remark}
Remark that ${z_k}^{n}$ descends to $X$ therefore all denominators of the rational numbers $b_{lk}$ must divide $n$.
\end{remark}

\subsection{Discrepancies}
Now, we describe some basic estimates on discrepancies associated to cyclic quotient singularities.

\begin{lemma} \label{lemdiscrepancy}
Let $X = \quotient{\Omega}{\Gamma}$ be a quotient with only cyclic quotient singularities $p_1, ..., p_r$, with isotropy groups $G_i$ such that $|G_i|=m_i$.
Let $K_{\widetilde{X}} = \pi^\ast K_{X} + \sum_i a_i E_i$, where the $a_i$ are the discrepancies. Then, for any $i$, we have $a_i \leq n(1 - \frac{1}{m_i}) - 1$.  
\end{lemma}
\begin{proof}
On each open chart $U_j$, we have, for any $k \in \left[|1,n\right|]$,
\begin{equation} \label{changecoordforms}
\pi^\ast (d z_k) = \sum_l \left[ \prod_{s\neq l} (u_s^j)^{b_{sk}} \right] (u_l^j)^{b_{lk} - 1} d u_l^j.
\end{equation}
Consequently, $\pi^\ast (dz_1 \wedge ... \wedge dz_n)$ can be written as $P(u_1^j, ..., u_k^j) du_1^j \wedge ... \wedge du_l^j$ for some $P \in \mathbb C[ u_1^j, ..., u_k^j]$. Since for each $s$, we have $b_{sj} \leq 1 - \frac{1}{m_i}$, we see from \eqref{changecoordforms} that in each monomial of $P$, each $u_i^j$ appears with degree at most $n (1 - \frac{1}{m_i}) - 1$.

Consequently, the pluricanonical form $\pi^\ast (dz_1 \wedge ... \wedge dz_n)^{\otimes m_i}$ vanishes at order at most $m_i \left[ n(1 - \frac{1}{m_i}) - 1\right]$ along $E_i$, if we see it as a local section of $K_{\widetilde{X}}^{\otimes m_i}$. This means exactly that $a_i \leq n(1 - \frac{1}{m_i}) - 1$.
\end{proof}


==> extension.tex <==
\section{Orbifold differential forms}\label{extension}

Our aim in the current section is to establish an extension result 
for orbifold differential forms (see Proposition~\ref{prop:extension}) which plays a key 
role in our strategy to prove Theorem~C. 


\subsection{Preliminaries on orbifold differential forms}
 The notions we are about to introduce in the current section originated in the 
 works of Campana, cf.~\cite{Cam04}. For a more thorough account of these
 preliminary constructions, including background and applications, 
 the reader could also consult~\cite{MR2860268},~\cite{Taji16},~\cite{CKT16} and~\cite{GT16}.
 
 


\begin{definition}\label{def:pair}
We define an orbifold pair $(X,D)$ by a normal, algebraic variety $X$ and 
a divisor $D = \sum_{i=1}^l d_i \cdot D_i$, with $d_i = (1- \frac{1}{a_i})$, where 
$a_i \in \mathbb N^+ \cup \{ \infty \}$ and each $D_i$ is a prime divisor. 

\end{definition}

We follows the usual convention that, for $a_i = \infty$, we have $(1- \frac{1}{a_i}) = 1$.

The pair $(X,D)$ in Definition~\ref{def:pair} is sometimes referred to as a pair with standard coefficients
(or a classical or integral orbifold pair).

With Definition~\ref{def:pair} at hand, given a pair $(X,D)$, one can naturally associate a notion of 
multiplicity to each irreducible component $D_i$ of $D$.

\begin{definition}
Let $(X,D)$ be an orbifold pair. we define the orbifold multiplicity $m_{D}(D_i)$ of each 
prime divisor $D_i$ as follows. 

$$
  m_D(D_i) := \left\{ 
    \begin{matrix}
      a_i & \text{, if $d_i\neq 1$ } \\
      \infty & \text{, if $d_i=1.$  }
    \end{matrix}
  \right.
  $$


\end{definition}

Our aim in now to introduce morphisms sensitive to the orbifold structure of $(X,D)$, but to do so 
we first need to define a notion for pullbacks of Weil divisors over normal varieties. 

\begin{definition}\label{def:pullback}
Let $f: Y\to X$ be a finite morphism of normal, algebraic varieties $X$ and $Y$. 
Let $D\subset X$ be a Weil divisor. We define 
$f^*(D)$ by the Zariski closure of the Weil divisor defined by $f^*(D|_{X_{\reg}})$.
\end{definition}

\medskip

We now turn to morphisms adapted to $(X,D)$. Such morphisms are guaranteed to 
exist whenever $X$ is smooth, thanks to Kawamata's covering constructions, 
cf.~\cite[Prop.~4.1.12]{Laz04-I}. 

\begin{definition}\label{def:adapted}
Let $(X,D)$ be an orbifold pair in Definition~\ref{def:pair}. We call a finite morphism 
$f: Y \to X$ of algebraic varieties $X$ and $Y$, strictly adapted (to $D$), if $Y$ is normal and 
$f^*(D_i) = a_i \cdot D'$, for some reduced divisor $D'$ in $Y$. 


\end{definition}


We can also consider collections of charts that are adapted to the orbifold 
structure of a given pair $(X,D)$. 

\begin{definition}[Orbifold structures]\label{def:structure}
Given an orbifold pair $(X,D)$, let $\{ U_{\alpha}\}_{\alpha}$ be a Zariski open covering of $X$. 
We call a collection $\mathcal C_{\alpha} = \{ (U_{\alpha}, f_{\alpha}, X_{\alpha} )\}_{\alpha}$ 
of triples $(U_{\alpha}, f_{\alpha}, X_{\alpha})$
consisting of strictly adapted morphisms $f_{\alpha}: X_{\alpha} \to (U_{\alpha}, D|_{U_{\alpha}})$, 
an orbifold structure (or strictly adapted orbifold structure) associated to $(X,D)$.

\end{definition}

\medskip


\begin{notation}
Given a coherent sheaf $\sF$ on a normal algebraic variety $X$, by $\Sym ^{[\bullet]}\sF$
we denote the reflexive hull $(\Sym^{\bullet}\sF)^{\vee\vee}$ of symmetric powers 
$\Sym^{\bullet}\sF$ of $\sF$. Furthermore, for a morphism of normal 
algebraic varieties $f: Y \to X$, we set $f^{[*]}\sF$ to denote $(f^*\sF)^{\vee \vee}$.

\end{notation}

We can now define a notion of sheaves of differential forms adapted to the orbifold 
structure of $(X,D)$. First, we need to fix some notations. 

\begin{notation}\label{not:orbi}
Let $\mathcal C_{\alpha}$ be an orbifold structure for the orbifold pair $(X,D)$.
Let $\{ D_{X_{\alpha}}^{ij} \}_{i, j}$ be the collection of prime divisors in $X_{\alpha}$ verifying the 
equality $\bigl(f^*(D_i)\bigr)_{\mathrm red}= \sum_j  D^{ij}_{X_{\alpha}}$. 
Let $X_{\alpha}^\circ$ denote the smooth locus of 
$(X_{\alpha}, f_{\alpha}^*(D))$ and $U_{\alpha}^\circ$ an open subset of 
the smooth locus of $(U_{\alpha}, D)$ such that $f_{\alpha}: X_{\alpha}^\circ\to U_{\alpha}^\circ$ is surjective.
\end{notation}

\begin{definition}\label{def:OrbiCot}
In the setting of Notation~\ref{not:orbi}, we define the 
orbifold cotangent sheaf $\Omega_{\mathcal C_{\alpha}}^{[1]}$ by the collection 
of reflexive, $\sO_{X_{\alpha}}$-module, coherent sheaves $\Omega^{[1]}_{(X_{\alpha}, f_{\alpha}, D)}$ 
uniquely determined as the coherent extension of the 
kernel of the sheaf morphism 

$$
f_{\alpha}^*\Omega^1_{U_{\alpha}^\circ} \big(  \log ( \ulcorner D   |_{U_{\alpha}^\circ} \urcorner) \big) 
   \longrightarrow \bigoplus \sO_{D_{X_{\alpha}^\circ}^{ij}},
$$
naturally defined by the residue map. 
\end{definition}


\begin{remark}
This is an instance of the notion of orbifolds sheaves adapted to a pair $(X,D)$.
These are $G_{\alpha}$-linearized, coherent sheaves on each $X_{\alpha}$
satisfying natural compatibility conditions, cf.~\cite[Sect.~2.6]{GT16}.
\end{remark}


\begin{example}\label{ex:OrbiCot}
Let $(X, D =\sum_{i=1}^l (1-\frac{1}{a_i})\cdot D_i)$ be an orbifold pair and $f_{\alpha}: X_{\alpha}\to U_{\alpha}$ 
 a single, strictly adapted chart in Definition~\ref{def:structure}.
Assume that the branch locus of $f_{\alpha}$ is divisorial and has simple normal crossing support. 
With this assumption, it follows that $X_{\alpha}$ is smooth. 
Furthermore, let us assume that $U_{\alpha}$ admits a coordinate system $(z_1, \ldots, z_n)$
such that $U_{\alpha}\cap D = \{ (z_1, \ldots, z_n) \; \big| \;  \prod_{i=1}^l z_i =0   \}$.
Assume that $w_1, \ldots , w_n$ is a coordinate system on $X_{\alpha}$ such that 

$$
f_{\alpha}: (w_1, \ldots, w_n) \mapsto (w_1^{a_1} , \ldots, w_l^{a_l}, w_{l+1}^{b_1}, \ldots, w_{l+k}^{b_k},
w_{l+k+1}, \ldots, w_n),
$$
for some $b_1, \ldots, b_k \in \mathbb N$.
Then, by definition, the sheaf $\Omega^1_{(X_{\alpha}, f_{\alpha}, D )}$
is the $\sO_{X_{\alpha}}$-module generated by 
$$
\langle    dw_1  , \ldots, dw_l,  (w^{b_1-1}_{l+1})\cdot dw_{l+1}, \ldots, (w^{b_k-1}_{l+k})\cdot dw_{l+k}, 
dw_{l+k+1}, \ldots, dw_n \rangle. 
$$

\end{example}

\medskip

\begin{definition}
Give any orbifold pair $(X,D)$ together with an orbifold structure 
$\mathcal C_{\alpha} =  \{ (U_{\alpha}, f_{\alpha}, X_{\alpha}) \}_{\alpha}$, 
we define the sheaf of symmetric orbifold differential forms $\Sym^{[\bullet]} \Omega^{[1]}_{\mathcal C_{\alpha}}$
by the collection of reflexive sheaves $\{ \Sym^{[\bullet]} \Omega^{[1]}_{(X_{\alpha}, f_{\alpha}, D)}  \}_{\alpha}$
on each $X_{\alpha}$.

\end{definition}

\medskip

\begin{notation}
Let $(X,D)$ be an orbifold pair. We shall denote by $\Sym^{[\bullet]}\Omega^{[1]}_X(*  D_{\red})$
the sheaf of symmetric rational differential forms with poles of arbitrary order along $D_{\red}$,
which is defined by:

$$
\lim_{\substack{\longrightarrow\\ m}} \Bigl(S^{[\bullet]} \Omega_X^{[1]} \otimes \sO_X(m\cdot D_{\red}) \Big)^{\vee\vee}.
$$

\end{notation}


Sometimes It is more convenient to work with a notion of symmetric differential forms, 
adapted to $(X,D)$, as a coherent sheaf on $X$ instead of $X_{\alpha}$. 
This is the purpose of the following definition. 


\begin{definition}
\label{def:CDiff}
Let $(X,D)$ be an orbifold pair equipped with an orbifold structure 
$\mathcal C_{\alpha} = \{ (U_{\alpha}, f_{\alpha}, X_{\alpha})  \}_{\alpha}$.
We define the sheaf of $\mathcal C$-differential forms $\Sym^{[\bullet]}_{\mathcal C} \Omega^{[1]}_X\log (D)$
to be the reflexive, coherent subsheaf of $\Sym^{[\bullet]} \Omega^{[1]}_X(*D_{\red})$, defined, at the level of 
presheaves, by the following property: 



\begin{IEEEeqnarray}{rCl}
\sigma \in \Gamma (U_{\alpha}, \Sym^{[\bullet]}_{\mathcal C} \Omega^{[1]}_X\log (D)) \; \; \Longleftrightarrow \;\;
   \sigma \in \Gamma(U_{\alpha}, S^{[\bullet]} \Omega^{[1]}_X(* D_{\red}) ) \; \; \text{and} \nonumber \\
    f^{[*]}_{\alpha}(\sigma) \in \Gamma (X_{\alpha}, \Sym^{[\bullet]} \Omega^{[1]}_{(X_{\alpha, f_{\alpha}, D})} ).\nonumber
\end{IEEEeqnarray}

\end{definition}



\begin{remark}
One can easily check that the notion of $\mathcal C$-differential forms in Definition~\ref{def:CDiff}
is independent of the choice of the orbifold structure $\mathcal C_{\alpha}$.
\end{remark}

\begin{remark}
Local calculations show that over $X_{\reg}$ the sheaf $\Sym_{\mathcal C}^{[\bullet]}\Omega^{[1]}_{X}\log(D)$ 
is locally free. More precisely, for every $x\in X_{\reg}$, there
exists an open neighbourhood $W_x\subset X_{\reg}$ with $W_x\cap D = \{ (z_1, \ldots, z_n) \; \big| \; \prod_{i=1}^l z_i =0  \}$ 
such that $\Sym^N_{\mathcal C}\Omega^1_{X_{\reg}}\log (D|_{\reg})$ is the $\sO_W$-module 
freely generated by 
$$
\langle \frac{dz_1^{m_1}}{z_1^{\lfloor m_1\cdot d_1 \rfloor}}, \ldots, \frac{dz_l^{m_l}}{z_l^{\lfloor m_l\cdot d_l \rfloor}},
     dz_{l+1}^{m_{l+1}}, \ldots, dz_n^{m_n}  \rangle, \;  \; \; \sum_{i=1}^n m_i = N,
$$
where $d_i= (1-\frac{1}{a_i})$.
\end{remark}


\subsection{An extension theorem for symmetric orbifold differential forms}
We are now ready to prove an extension result for orbifold differential forms,
which can be interpreted as an
orbifold version of~\cite[Prop.~3.1]{GKK08}.

\begin{proposition}
\label{prop:extension}
Let $U\subseteq \mathbb C^n$ be a normal, algebraic subset. Assume 
that there is a smooth algebraic subset $V\subseteq \mathbb C^n$
and a finite group $G$ acting freely in codimension one such that $U\cong V/G$. 
Let $\pi: \wtilde U \to U$ be a strong log-resolution of $U$ with $E\subseteq \Exc(\pi)$ being the 
maximal reduced exceptional divisor. Then, for every $m\in \mathbb N$, the
coherent sheaf 
\begin{equation}\label{def:sheaf}
\sG: = \pi_*\Big( \Sym^m_{\mathcal C} \Omega^1_{\wtilde U}\log \big( (1-\frac{1}{| G |})\cdot E  \big)   \Big)
\end{equation}
is reflexive. 

\end{proposition}


\begin{proof}
Let $f: V\to U$ denote the finite map encoding the isomorphism $U \cong V/G$
and set $\wtilde V$ to be the normalization of the fibre product $V\times_U \wtilde U$ with 
the resulting commutative diagram:



  $$
  \xymatrix{
    \wtilde V \ar[rrr]^{\wtilde f, \; \text{finite}} \ar[d]_{\wtilde \pi} &&& \wtilde U \ar[d]^{\pi} \\
      V \ar[rrr]^{f \;=\; \cdot/G}     &&& U
  }
  $$

 Note that $\wtilde f$ is a composition of the finite map $V \times_U \wtilde U\to \wtilde U$, which is 
of degree $|G|$, and its normalization. Therefore $\deg(\wtilde f) = | G |$.


Now, as the problem is local, 
to prove the reflexivity of the sheaf $\sG$ (\ref{def:sheaf}),
it suffices to show that the naturally defined map 

\begin{equation}\label{eq:surject}
\Gamma\big(\wtilde U, \Sym^m_{\mathcal C} \Omega^1_{\wtilde U} \log \Big( ( 1-\frac{1}{| G |}  ) \cdot E  \Big) \big)
       \longrightarrow    \Gamma \big(\wtilde U\backslash \Exc(\pi),  \Sym^m \Omega^1_{\wtilde U} \big)
\end{equation}
 is surjective. 
 
 To this end, let $\sigma \in \Gamma(U, \Sym^{[m]} \Omega^{[1]}_U)$ 
 be the section defined by $\wtilde \sigma \in \Gamma\big( \wtilde U\backslash \Exc(\pi) ,\Sym^m \Omega^1_{\wtilde U}\big)$.
 Let $\sigma_V = f^{[*]}\sigma \in \Gamma(V, \Sym^m \Omega^1_V)$.
  As $\sigma_V$ is regular, we have 
  $$
   \wtilde \pi^* f^{[*]} (\sigma) =  \wtilde \pi^*(\sigma_V)\in \Gamma(\wtilde V ,\Sym^{[m]}\Omega^{[1]}_{\wtilde V}).
  $$
  Viewing $\wtilde \sigma$ as an element of $\Gamma\big(\wtilde U, \Sym^m \Omega^1_{\wtilde U}(* E)\big)$, 
  and thanks to the commutativity of the diagram above, we have
  
  \begin{equation}\label{eq:include}
   \wtilde f^*(\sigma)
   \in \Gamma(\wtilde V , \Sym^{[m]}\Omega^{[1]}_{\wtilde V}).
  \end{equation} 

Now, set $\{E_i$\} to be the set of irreducible components of $E$ and let 
$$
E' = \sum (1- \frac{1}{a_i})\cdot E_i
$$
be the divisor with respect to which $\wtilde f : \wtilde V \to \wtilde U$ is strictly adapted 
to the orbifold pair $(\wtilde U, E')$
(cf.~Definition~\ref{def:adapted}).
Note that, by construction, we have:

\begin{enumerate}
\item \label{item:1} For each $i$, the inequality $a_i \leq | G |$ holds. 
\item $\Omega^{[1]}_{\wtilde V} = \Omega^{[1]}_{(\wtilde V, \wtilde f, E')}$ (cf.~Example~\ref{ex:OrbiCot}).
\end{enumerate}

Therefore, thanks to (\ref{eq:include}) we have, by the definition of symmetric $\mathcal C$-differential forms, 
that $\sigma \in \Gamma\big(\wtilde U, \Sym^m_{\mathcal C} \Omega^1_{\wtilde U} \log (E')\big)$. In 
particular, it follows that  
the map

$$
\Gamma\big(\wtilde U,  \Sym^m_{\mathcal C} \Omega^1_{\wtilde U}\log (E')   \big)     \longrightarrow  
    \Gamma \big( \wtilde U\backslash \Exc(\pi), \Sym^m\Omega^1_{\wtilde U}    \big)$$

is a surjection.

On the other hand, thanks to the inequality $a_i \leq |G|$ in~\ref{item:1}, we have

$$
\Sym^m_{\mathcal C} \Omega^1_{\wtilde U}\log (E') \subseteq 
        \Sym^m_{\mathcal C} \Omega^1_{\wtilde U} \log\big(  (1- \frac{1}{|G|})\cdot E \big).
$$
 The surjectivity of the map~(\ref{eq:surject}) now follows. 
\end{proof}





We conclude this section by pointing out that
one can easily verify that the extension result in Proposition~\ref{prop:extension} holds for any 
resolution of $U$.
